Automatic Relation-aware Graph Network Proliferation

Graph neural architecture search has sparked much attention as Graph Neural Networks (GNNs) have shown powerful reasoning capability in many relational tasks. However, the currently used graph search space overemphasizes learning node features and neglects mining hierarchical relational information. Moreover, due to diverse mechanisms in the message passing, the graph search space is much larger than that of CNNs. This hinders the straightforward application of classical search strategies for exploring complicated graph search space. We propose Automatic Relation-aware Graph Network Proliferation (ARGNP) for efficiently searching GNNs with a relation-guided message passing mechanism. Specifically, we first devise a novel dual relation-aware graph search space that comprises both node and relation learning operations. These operations can extract hierarchical node/relational information and provide anisotropic guidance for message passing on a graph. Second, analogous to cell proliferation, we design a network proliferation search paradigm to progressively determine the GNN architectures by iteratively performing network division and differentiation. The experiments on six datasets for four graph learning tasks demonstrate that GNNs produced by our method are superior to the current state-of-the-art hand-crafted and search-based GNNs. Codes are available at https://github.com/phython96/ARGNP.

==> tables/statistic.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[ht]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{2.0 mm}
    \caption{
        \textbf{Summary statistics of six datasets. }
    }
    \label{statistic}
    \begin{tabular}{@{}ccccccc@{}}
    \toprule
                & \textbf{Node Level} & \multicolumn{4}{c}{\textbf{Graph Level}}          & \textbf{Edge Level} \\ \cmidrule(l){2-2} \cmidrule(l){3-6} \cmidrule(l){7-7}
                & \textbf{CLUSTER}    & \textbf{ZINC}       & \textbf{CIFAR10}      & \textbf{ModelNet10}       & \textbf{ModelNet40}       & \textbf{TSP}          \\ \midrule
    Graphs      &  12K                &  12K                &  60K                  & 5,000                     & 48,000                    &  12K                  \\
    Nodes       &  41-190             &  9-37               &  85-150               & 2,048                     & 2,048                     &  50-500               \\
    Total Nodes &  1,406,436          &  277,864            &  7,058,005            & ---                       & 98,304,000                &  3,309,140            \\ 
    \bottomrule
    \end{tabular}
\end{table*}
